A Comparative Exploration of ML Techniques for Tuning Query Degree of Parallelism

There is a large body of recent work applying machine learning (ML) techniques to query optimization and query performance prediction in relational database management systems (RDBMSs). However, these works typically ignore the effect of \textit{intra-parallelism} -- a key component used to boost the performance of OLAP queries in practice -- on query performance prediction. In this paper, we take a first step towards filling this gap by studying the problem of \textit{tuning the degree of parallelism (DOP) via ML techniques} in Microsoft SQL Server, a popular commercial RDBMS that allows an individual query to execute using multiple cores. In our study, we cast the problem of DOP tuning as a {\em regression} task, and examine how several popular ML models can help with query performance prediction in a multi-core setting. We explore the design space and perform an extensive experimental study comparing different models against a list of performance metrics, testing how well they generalize in different settings: $(i)$ to queries from the same template, $(ii)$ to queries from a new template, $(iii)$ to instances of different scale, and $(iv)$ to different instances and queries. Our experimental results show that a simple featurization of the input query plan that ignores cost model estimations can accurately predict query performance, capture the speedup trend with respect to the available parallelism, as well as help with automatically choosing an optimal per-query DOP.

==> todolist.tex <==
\section*{TODO List}
\zhiwei{Here is the TODO list regarding the rest of the work needed to be done for the paper. I briefly discuss about different items and highlight the approximated time required for each of the task. Regarding the importance and the priority of different tasks, we need to discuss to  fully determine them.}

\todo{
\begin{itemize}
   \item Variance Analysis: find an example query executed multiple times at the same DOP showing large variance in execution time of the {\em same physical operator} within the query plan, for the purpose of quantitively justifying why the model relying on operator-level execution latency info is not likely work for our problem. [1-2 hours]
%   \item Featurization Analysis: I consider this as one of the most important task remaining to be done which I overlooked before (many apologies). While I have not seen any of the justification of different ways of featurization in recent ML for DBMS work, I do think it is very important since it's tied to other things such as model effectiveness/efficiency, easiness of interpretability study. Many ideas regarding this part have come to my mind: 
%   \begin{itemize}
%   	\item currently I am not including the "input" estimate for each physical operators (except for the scan operator) since it is not directly included in the plan, but including it should be important and straightforward, so I am planning to include that [$\sim 2 $hours]\revise{[DONE]}; 
%	\item an simple analysis should be done to see how many different {\em composite keys} 
%	(e.g.,  $$<\text{physical\_op\_type}>\_<\text{if parallel}>$$
%	$$\_<\text{batch or row}>\_<\text{adaptive or not}> ...$$)) show up in the different query set, this will give us some intuition regarding the choice of featurization  [$\sim 2 $hours] \revise{[DONE] (53 different keys in total, top\_parallel\_row in tpc-h not in tpc-ds)}; 
%	\item Consider three featurization alternatives (for numerical values): 1) using {\em ONLY} resource cost estimate from the query optimizer as features; 2) using {\em ONLY} estimated input and output info from constructed from \textit{estimated cardinalities} as features; 3) use both 1) and 2) [ $> 2$ days] \revise{[DONE]} (the implementation is done. Now featurization focuses on composite-key representation with children operator inputs and structural info being added)
%   \end{itemize}
%   \item Tuning XGBoost on different training dataset [$\sim 1$ day]
   \item Interpretability \& ablation study [$\sim 2$ days]
   \item Finish the Write-up  [$\sim 1$ day]
   \item Characterization changed with considering parallel plans only \revise{[DONE]} \& reasoning about the architecture \& hyper-parameter choices of MLP [$\sim 4 $hours]
%   \item Re-do visualization if time permits on Python [$\sim 1$ day]
	\item Fix the inconsistency regarding the notation used using Macro
\end{itemize}}

